Unveiling the Ignorance of MLLMs: Seeing Clearly, Answering Incorrectly

Multimodal Large Language Models (MLLMs) have displayed remarkable performance in multi-modal tasks, particularly in visual comprehension. However, we reveal that MLLMs often generate incorrect answers even when they understand the visual content. To this end, we manually construct a benchmark with 12 categories and design evaluation metrics that assess the degree of error in MLLM responses even when the visual content is seemingly understood. Based on this benchmark, we test 15 leading MLLMs and analyze the distribution of attention maps and logits of some MLLMs. Our investigation identifies two primary issues: 1) most instruction tuning datasets predominantly feature questions that 'directly' relate to the visual content, leading to a bias in MLLMs' responses to other indirect questions, and 2) MLLMs' attention to visual tokens is notably lower than to system and question tokens. We further observe that attention scores between questions and visual tokens as well as the model's confidence in the answers are lower in response to misleading questions than to straightforward ones. To address the first challenge, we introduce a paired positive and negative data construction pipeline to diversify the dataset. For the second challenge, we propose to enhance the model's focus on visual content during decoding by refining the text and visual prompt. For the text prompt, we propose a content guided refinement strategy that performs preliminary visual content analysis to generate structured information before answering the question. Additionally, we employ a visual attention refinement strategy that highlights question-relevant visual tokens to increase the model's attention to visual content that aligns with the question. Extensive experiments demonstrate that these challenges can be significantly mitigated with our proposed dataset and techniques.

==> sec/abstract_bak.tex <==
\begin{abstract}
\textbf{M}ultimodal \textbf{L}arge \textbf{L}anguage \textbf{M}odels (MLLMs) have shown remarkable performance in multimodal tasks, particularly in visual comprehension. However, we reveal that MLLMs can generate incorrect answers even when they accurately understand visual content (for example, character and counting). 
In this paper, we investigate this phenomenon by introducing a benchmark and new metrics to explore the correctness of MLLM's responses to questions when understanding the visual content. We also analyze the attention mechanisms and logit distribution. We identify two primary issues: 1) most fine-tuning datasets predominantly feature questions aimed at understanding visual content, leading to a bias in MLLMs' responses to misleading questions, and 2) MLLMs’ attention to visual tokens is notably lower than to system and question tokens. We further observe that attention scores between question and visual tokens and model confidence in correct answers are lower in response to misleading questions than to straightforward ones. To address the first challenge, we introduce a paired positive and negative data construction pipeline to diversify the dataset and mitigate the influence of bias on MLLM responses. For the second challenge, we propose to enhance the model's focus on visual content during decoding by refining the text and visual prompt. For the text prompt, we propose a content-guided refinement strategy that first performs preliminary visual content analysis to generate structured information before answering the question. Additionally, we employ a visual attention refinement strategy that highlights question-relevant visual tokens to increase the model’s attention to visual content that aligns with the question. Extensive experiments demonstrate that these challenges can be significantly mitigated with our proposed dataset and techniques. The benchmark, training set, and code will be available.
\end{abstract}

==> sec/intro_bak.tex <==
\section{Introduction}
\textbf{M}ultimodal \textbf{L}arge \textbf{L}anguage \textbf{M}odels (MLLMs) have garnered significant attention due to their impressive capabilities in addressing diverse multimodal tasks, particularly in visual comprehension and reasoning~\cite{team2023gemini, alayrac2022flamingo, he2024efficient}. Despite these strengths, MLLMs sometimes produce responses that deviate from the image content, resulting in what is termed ``hallucinations." Previous studies like MME~\cite{mme}, POPE~\cite{li-etal-2023-evaluating}, ConBench~\cite{zhang2024unveiling}, and NaturalBench~\cite{li2024naturalbench} examine MLLM response accuracy under image or text perturbations. However, they do not distinguish between two causes of incorrect responses: 1) MLLMs do not understand the content of the image, and 2) MLLMs understand the content of the image but answer incorrectly. In this paper, we target the latter—instances where MLLMs, despite fully understanding the visual content, still respond inaccurately (as illustrated in Fig.~\ref{cover_figure} (a)). Our findings suggest that subtle phrasing in questions can introduce biases that hinder MLLMs from leveraging their understanding accurately. This raises two critical questions for our research: \textit{1) Why does the model understand the visual content but provide incorrect answers? 2) How can we correct this error-prone behavior of MLLMs?}

To explore this phenomenon, we introduce the \textbf{M}LLM \textbf{M}isresponses despite \textbf{V}isual \textbf{U}nderstanding (MMVU) benchmark, as shown in Fig.~\ref{benchmark_case}. Each sample is manually labeled with one of 12 types of questions, accompanied by paired positive and negative questions. Positive questions are designed to directly and objectively inquire about the observable content within an image, such as its types, attributes, poses, movements, or scenes, based on the actual and verifiable elements present, without introducing hypothetical alterations, irrelevant details, or erroneous premises. These questions aim to evaluate the model's comprehension of the visual content. In contrast, negative questions often involve hypothetical modifications, irrelevant descriptions, or incorrect assumptions about the image, which can lead to confusion or misinterpretation of the visual information. As a result, such questions may induce incorrect responses, as they present scenarios that do not align with the image’s actual content. For instance, a positive question might ask, ``\textit{What animal is in the image?}" while a negative question might inquire, ``\textit{What color is the elephant in the image?}" if no elephant is present. To ensure MLLMs select the most appropriate response based on their understanding of the visual content, we design multiple-choice questions with correct answers and carefully crafted distractors that include explanatory content, reducing the reliance on random or incorrect guesses. Additionally, we propose novel metrics to measure the likelihood of a MLLM's failure when influenced by a negative question, despite its comprehension of the visual content. 

We evaluate 14 leading MLLMs on the MMVU benchmark, as shown in Tab.~\ref{tab:mma_benchmark}. We also analyze the attention maps and logits of some MLLMs when faced with different types of questions during the decoding process, as depicted in Fig.~\ref{fig: analysis}. Our findings reveal that most MLLMs respond unsatisfactorily to negative questions, demonstrating a biased response toward positive answers regardless of the question type. This phenomenon can be attributed to two main issues: 1) the fine-tuning dataset is predominantly composed of positive question-answer pairs, leading MLLMs to favor positive responses due to the scarcity of negative samples, and 2) there is an unbalanced distribution of attention, with models prioritizing system and question tokens while significantly neglecting visual tokens. We further observe that attention scores between question and visual tokens and model confidence in correct answers are lower in response to negative than positive questions.

To address the first issue, we introduce a data construction pipeline that extracts a wide range of visual information from images, such as text, numbers, objects, attributes, relationships, and contextual elements at both local and global levels. Based on this information, we construct paired positive and negative samples to form the MMVU-training dataset, consisting of 112k pairs. 
For the second issue, we aim to enhance the model's attention to visual content during decoding by implementing two key strategies:
1) Content-guided refinement (CGR). This method employs a two-step reasoning process where the model first extracts detailed information from the image and then formulates responses based on this analysis alongside the visual content. 2) Visual attention refinement (VAR). To guide the MLLM in focusing on critical visual features relevant to the question, we extract attention scores and apply a mask to help focus on significant areas while masking less important ones.

In summary, our contributions are as follows: \textbf{1)} We identify and analyze the issue of MLLMs generating incorrect answers despite accurate visual comprehension, attributing this to specific underlying biases. We introduce the MMVU benchmark and new metrics to evaluate MLLMs’ comprehension and resilience to negative questions. \textbf{2)} We introduce a data construction pipeline that generates paired positive and negative samples to enhance the model's robustness to negative questions. Furthermore, we propose CGR and VAR strategies to optimize the model's focus on relevant visual content and enhance response accuracy. \textbf{3)} Extensive experiments reveal that our dataset and strategies effectively mitigate the susceptibility of MLLMs to negative questions.


==> tables/finetune_mmr.tex <==
\begin{table*}
    \centering
    \caption{Comparison to state-of-the-art MLLMs on the MMR benchmark. $^\mathsection$We evaluate the officially released checkpoint by ourselves. Abbreviations: Char/Num. (Character/Number), Pres. (Presence), Color/Tex. (Color/Texture), Num. (Number), Shape (Shape), Posture (Posture), Pos. (Position), Abstract. (Abstract Knowledge), Concrete. (Concrete Knowledge), Expert (Expertise), Act. (Activity), Rel. (Relationships). $\uparrow$: higher is better, $\downarrow$: lower is better.}
    \vspace{0.3em}
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.05}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{lccccccccccccc}
            \specialrule{1.5pt}{0pt}{0pt}
            % \rowcolor[HTML]{EFEFEF}
            % & \multicolumn{1}{c|}{Char-Level} & \multicolumn{6}{c|}{Phrase-Level} & \multicolumn{5}{c|}{Sentence-Level} & Avg. \\ \cline{2-14}
            \rowcolor[HTML]{EFEFEF}
             Method & Char/Num & Pres. & Color/Tex & Num. & Shape & Posture & Pos. & Abstract. & Concrete. & Expert. & Act. & \multicolumn{1}{c}{Rel.} &  Avg. RA $\uparrow$\\
            \hline
            Random &25 &25 &25 &25 &25 &25 &25 &25 &25 &25 &25 &25 &25\\
            GPT4o~\cite{gpt4v} &76.83 &74.70 &67.74 &38.27 &76.39 &78.57 &49.30 &72.06 &70.31 &53.85 &74.44 &43.66 &65.06\\ 
            Gemini-1.5-Pro~\cite{team2023gemini} &47.56 &36.14 &41.94 &23.46 &43.06 &40.48 &15.49 &60.29 &56.25 &32.31 &50.00 &28.17 &39.53\\ 
            Qwen-VL-max-0809~\cite{bai2023qwenvl} &67.07 &60.87 &61.29 &34.48 &76.00 &62.07 &42.86 &69.57 &72.88 &67.74 &70.73 &54.55 &63.36\\
            Claude3.5-Sonnet-0620~\cite{anthropic2024claude} &64.63 &53.01 &66.13 &38.27 &56.94 &67.86 &38.03 &64.71 &64.06 &44.62 &67.78 &35.21 &55.32 \\
            LLaVA-OneVision-7B~\cite{liu2023llava} &62.20 &67.47 &70.97 &41.98 &58.33 &70.24 &49.30 &77.94 &71.88 &35.38 &75.56 &42.25 &60.58 \\
            Ovis1.6-Gemma2-9B~\cite{ai2024yi} &71.95 &74.70 &69.35 &58.02 &65.28 &76.19 &57.75 &77.94 &68.75 &47.69 &75.56 &52.11 &66.74 \\
            InternVL2-8B~\cite{chen2024far} &46.34 &65.06 &53.23 &33.33 &56.94 &53.57 &39.44 &61.76 &65.63 &29.23 &66.67 &21.13 &49.72\\
            MiniCPM-2.6V~\cite{viscpm} &69.51 &72.29 &69.35 &48.15 &51.39 &73.81 &45.07 &70.59 &71.88 &38.46 &80.00 &35.21 &61.14\\
            Cambrian-8B~\cite{wang2023cogvlm} &35.37 &60.24 &41.94 &40.74 &41.67 &57.14 &39.44 &44.12 &42.19 &24.62 &51.11 &28.17 &42.89 \\
            Idefics3-8B-Llama3~\cite{laurençon2024matters} &57.32 &61.45 &61.29 &43.21 &69.44 &64.29 &40.85 &61.76 &64.06 &30.77 &68.89 &36.62 &55.43 \\
            Pixtral-12B-2409~\cite{sun2023aligning} &48.78 &65.06 &66.13 &49.38 &50.00 &54.76 &56.34 &61.76 &65.63 &24.62 &66.67 &39.44 &54.31\\
            VILA1.5-13B~\cite{lu2024deepseek} &14.63 &30.12 &35.48 &12.35 &27.78 &42.86 &8.45 &29.41 &29.69 &16.92 &43.33 &14.08 &25.76 \\
            Llama3.2-11B-Vision-Instruct~\cite{ye2023mplugowl2} &64.63 &81.93 &80.65 &53.09 &70.83 &75.00 &56.34 &72.06 &76.56 &27.69 &82.22 &52.11 &66.63 \\
            Phi3.5-Vision-Instruct~\cite{abdin2024phi3} &54.88 &53.01 &61.29 &37.04 &58.33 &55.95 &35.21 &60.29 &64.06 &29.23 &68.89 &38.03 &51.62\\
            \specialrule{1.5pt}{0pt}{0pt}\\
        \end{tabular}
    }
    \vspace{-10pt}
    \label{tab:mma_benchmark}
\end{table*}
